ConflictBank: A Benchmark for Evaluating the Influence of Knowledge Conflicts in LLM

Large language models (LLMs) have achieved impressive advancements across numerous disciplines, yet the critical issue of knowledge conflicts, a major source of hallucinations, has rarely been studied. Only a few research explored the conflicts between the inherent knowledge of LLMs and the retrieved contextual knowledge. However, a thorough assessment of knowledge conflict in LLMs is still missing. Motivated by this research gap, we present ConflictBank, the first comprehensive benchmark developed to systematically evaluate knowledge conflicts from three aspects: (i) conflicts encountered in retrieved knowledge, (ii) conflicts within the models' encoded knowledge, and (iii) the interplay between these conflict forms. Our investigation delves into four model families and twelve LLM instances, meticulously analyzing conflicts stemming from misinformation, temporal discrepancies, and semantic divergences. Based on our proposed novel construction framework, we create 7,453,853 claim-evidence pairs and 553,117 QA pairs. We present numerous findings on model scale, conflict causes, and conflict types. We hope our ConflictBank benchmark will help the community better understand model behavior in conflicts and develop more reliable LLMs.

==> table/data_details.tex <==
\begin{table}[t]
\centering
\small
\begin{NiceTabular}{lcccc}
\toprule
\textbf{Mode}                    & \textbf{Samples}    & \textbf{Doc-Token}     & \textbf{\#Questions}       & \textbf{\#Entities}      \\
\midrule
\textbf{Fact}            & 2,513,403
                 & 1.24B      & -       & -        \\
\textbf{Misinformation}            & 2,524,579
                 & 1.24B      & -       & -          \\
\textbf{Temporal}            & 2,463,521
       & 1.45B     & -       & -      \\
\textbf{Semantic}            & 2,471,950 & 1.22B      & -       & -         \\ \midrule
\textbf{Total}            & 9,973,453 & 5.15B      & -       & -    \\
\bottomrule
\end{NiceTabular}
\caption{Statistics of our datasets.  \#Facts and \#Answers represent
the average number of facts and answers within the subject and question, respectively.}
\label{tab:data-stats}
\end{table}

==> table/inconsistent_rate.tex <==
\begin{table}[t]
\centering
\small
\begin{NiceTabular}{lccc}
\toprule
\textbf{Model}                    & \textbf{Without}    & \textbf{With}     & \textbf{Inconsist.}          \\
\midrule
\textbf{Fact}            & 2,513,403
                 & 1.24B      & -              \\
\textbf{Fact}            & 2,513,403
                 & 1.24B      & -              \\
\textbf{Fact}            & 2,513,403
                 & 1.24B      & -              \\
\textbf{Fact}            & 2,513,403
                 & 1.24B      & -              \\ 
\bottomrule
\end{NiceTabular}
\caption{Number of final examples for each LLM.
The difference between LLMs is due to their different outputs going through the framework. Answer inconsistency rate is the intersection set between the situation 1 and situation 2.}
\label{tab:data-stats}
\end{table}

==> table/model_information.tex <==
\begin{table}[!htbp]
    \centering
    \small
    \begin{tabular}{lll}
    \toprule
   \textbf{Model name in our paper} &\hspace{0.5pt}& \textbf{Model card in HuggingFace/OpenAI}\\
   \midrule
   \midrule
      Qwen1.5-0.5B   && Qwen/Qwen1.5-0.5B
      \\\midrule
      Qwen1.5-1.8B   && Qwen/Qwen1.5-1.8B
      \\\midrule
      Qwen1.5-4B   && Qwen/Qwen1.5-4B
      \\\midrule
      Qwen1.5-7B   && Qwen/Qwen1.5-7B
      \\\midrule
      Llama2-7b   && meta-llama/Llama-2-7b-hf
      \\\midrule
      Llama2-13b   && meta-llama/Llama-2-13b-hf
      \\\midrule
      Llama2-70b   && meta-llama/Llama-2-70b-hf 
      \\\midrule
      Llama3-8B   && meta-llama/Meta-Llama-3-8B
      \\\midrule
      Llama3-70B   && meta-llama/Meta-Llama-3-70B
      \\\midrule
      gemma-2b   && google/gemma-2b
      \\\midrule
      gemma-7b   && google/gemma-7b\\
        \bottomrule
    \end{tabular}
    \vspace{0.5em}
    \caption{Mapping between the model name in our paper and the exact model card name in HuggingFace. 
    %\ryan{double check this}
    }
    \label{tab:map between name and model cards}
\end{table}


==> table/prompt.tex <==
\begin{figure*}[ht]
    \centering
    \footnotesize
    \begin{tabularx}{\linewidth}{|X|}
    \toprule
        \textbf{Task}: Resolve semantic conflicts in descriptions involving the same terms used for different roles, due to polysemy. Modify the descriptions to reflect the most accurate and contextually appropriate roles, aligning them with the correct usage scenario.\\
        \textbf{Objective}: To accurately align and correct descriptions of terms that are used ambiguously across different contexts. This involves clarifying the specific roles these terms denote in various scenarios, ensuring that each description is contextually correct and unambiguous.\\
        \textbf{Example}:\\
        - Correct Claim: Franck Dupont holds the position of conseiller municipal de Zouafques.\\
        - Conflicting Claim: Franck Dupont holds the position of Governor of Taraba State.\\
        - Original Description for "Franck Dupont": French politician.\\
        - Description for "Governor of Taraba State": Political position in Nigeria.\\
        - Task: Modify the description to modify the usage of "Franck Dupont" by aligning it with a role appropriate for "Governor of Taraba State".\\
        - Modified Description for "Franck Dupont": Nigerian politician.\\
        \textbf{Template for Generating Descriptions}: \\
        - Correct Claim: \{correct\_pair\} \\
        - Conflicting Claim: \{conflict\_pair\} \\
        - Original Description for "\{subject\}": \{subject\_description\} \\
        - Description for "\{replaced\_object\}": \{object\_description\} \\
        - Task: Modify the description to modify the usage of "\{subject\}" by aligning it with a role appropriate for "\{replaced\_object\}". \\
        - Modified Description for "\{subject\}": [Only return the answer] \\
    \bottomrule
    \end{tabularx}
    \caption{Prompt on  LLaMA-3-70b-instruct for generating semantic descriptions to reflect the most accurate and contextually appropriate roles, aligning them with the correct usage scenario.}
    \label{fuck}
\end{figure*}



\begin{table*}[t!]
\resizebox{\linewidth}{!}{
    \centering
\begin{tabular}{l|l}
\toprule

\textbf{News}               & 
\begin{tabular}[c]{@{}l@{}}
Based on the provided description, craft a news report that offers well-researched and \\substantiated evidence for the statement. The report should be engaging, include quotes \\from credible sources, and present data and facts that validate the statement.\\

\end{tabular}          \\ \midrule

\textbf{Wikipedia}               & 
\begin{tabular}[c]{@{}l@{}}
Following the provided description, create a Wikipedia entry that systematically presents \\comprehensive evidence for the statement. The entry should be informative, well-structured,\\ and include references to credible sources that substantiate the statement.

\end{tabular}          \\ \midrule

\textbf{Books}               & 
\begin{tabular}[c]{@{}l@{}}
Utilizing the provided description, write a book narrative that intricately weaves in detailed \\evidence supporting the statement. The narrative should be rich in context, offer deep insights,\\ and use storytelling to elucidate the facts that back the statement.\\ 
\end{tabular}  \\ \midrule

\textbf{Prompt}               & 
\begin{tabular}[c]{@{}l@{}}
    \textbf{<Instruction>} \\
    \textbf{Description for \{subject\}}: \{subject\_description\} \\
    \textbf{Description for \{replaced\_object\}}: \{object\_description\} \\
    \textbf{Claim}: \{claim\} \\
    \textbf{Evidence}:\\
\end{tabular}  \\ 

\bottomrule
\end{tabular}}
    \caption{\textbf{Default evidence generation:} Prompt on \textsc{LLaMA-3-70b-instruct} for generating evidence based on the correct claim and its corresponding description. \textbf{<Instruction>} is randomly chosen from \textbf{News}, \textbf{Wikipedia} and \textbf{Books}.}
    % \vspace{-0.5em}
    \label{tb:case-study}
\end{table*}



\begin{table*}[t!]
\resizebox{\linewidth}{!}{
    \centering
\begin{tabular}{l|l}
\toprule

\textbf{News}               & 
\begin{tabular}[c]{@{}l@{}}
Based on the provided description, compose a news article that introduces a narrative \\aligning with the given claim, incorporating fictional interviews, events, and data. Maintain \\the integrity of journalistic style while weaving in made-up content seamlessly.\\

\end{tabular}          \\ \midrule

\textbf{Wikipedia}               & 
\begin{tabular}[c]{@{}l@{}}
Based on the provided description, construct a Wikipedia entry that outlines a series of \\events, studies, and references that are fictional but support the given claim. Ensure the \\entry maintains the formal tone and structure of a real Wikipedia article.\\

\end{tabular}          \\ \midrule

\textbf{Books}               & 
\begin{tabular}[c]{@{}l@{}}
Using the provided description as a foundation, craft a section of a book narrative that \\subtly introduces elements that support the given claim. Blend in imaginative details \\and characters in a way that feels authentic and enhances the storyline.\\ 
\end{tabular}  \\ \midrule

\textbf{Prompt}               & 
\begin{tabular}[c]{@{}l@{}}
    \textbf{<Instruction>} \\
    \textbf{Description for \{subject\}}: \{subject\_description\} \\
    \textbf{Description for \{replaced\_object\}}: \{replaced\_object\_description\} \\
    \textbf{Claim}: \{claim\} \\
    \textbf{Evidence}:\\
\end{tabular}  \\ 

\bottomrule
\end{tabular}}
    \caption{Prompt on LLaMA-3-70b-instruct for generating evidence based on the misinformation claim and its corresponding description. \textbf{<Instruction>} is randomly chosen from \textbf{News}, \textbf{Wikipedia} and \textbf{Books}.}
    % \vspace{-0.5em}
    \label{tb:case-study}
\end{table*}



\begin{table*}[t!]
\resizebox{\linewidth}{!}{
    \centering
\begin{tabular}{l|l}
\toprule

\textbf{News}               & 
\begin{tabular}[c]{@{}l@{}}
Based on the provided descriptions, please write a news report. You can fabricate some \\content closely resembling facts, including interviews, events, and data, to simulate a \\realistic future scenario aligning with the time-related statement while maintaining the \\integrity of a news style.\\

\end{tabular}          \\ \midrule

\textbf{Wikipedia}               & 
\begin{tabular}[c]{@{}l@{}}
Based on the provided description, construct a Wikipedia entry. Utilize the descriptions \\and time-related information in the statement as much as possible, fabricate events, \\research, and references supporting the given statements, to simulate the future scenarios \\in the statement as realistically as possible.\\

\end{tabular}          \\ \midrule

\textbf{Books}               & 
\begin{tabular}[c]{@{}l@{}}
 Using the provided description, write a narrative for a book, with a focus on the temporal \\information in the statement. Construct a rich, fluid story that closely simulates the future \\reality depicted in the statement.\\ 
\end{tabular}  \\ \midrule

\textbf{Prompt}               & 
\begin{tabular}[c]{@{}l@{}}
    \textbf{<Instruction>} \\
    \textbf{Description for \{subject\}}: \{subject\_description\} \\
    \textbf{Description for \{replaced\_object\}}: \{replaced\_object\_description\} \\
    \textbf{Claim}: \{claim\} \\
    \textbf{Evidence}:\\
\end{tabular}  \\ 

\bottomrule
\end{tabular}}
    \caption{Prompt on LLaMA-3-70b-instruct for generating evidence based on the temporal claim and its corresponding description. \textbf{<Instruction>} is randomly chosen from \textbf{News}, \textbf{Wikipedia} and \textbf{Books}.}
    % \vspace{-0.5em}
    \label{tb:case-study}
\end{table*}


\begin{table*}[t!]
\resizebox{\linewidth}{!}{
    \centering
\begin{tabular}{l|l}
\toprule
\textbf{News}               & 
\begin{tabular}[c]{@{}l@{}}
Based on the provided description, compose a news article that introduces a narrative \\aligning with the given claim, incorporating fictional interviews, events, and data. \\Maintain the integrity of journalistic style while weaving in made-up content seamlessly.\\
Description for \{semantic\_subject\}: \{semantic\_subject\_description\} \\
Description for \{object\}: \{replaced\_object\_description\} \\
Claim: \{claim\} \\
Evidence:\\
\end{tabular}          \\ \midrule

\textbf{Wikipedia}               & 
\begin{tabular}[c]{@{}l@{}}
Based on the provided description, construct a Wikipedia entry that outlines a series of \\events, studies, and references that are fictional but support the given claim. Ensure \\the entry maintains the formal tone and structure of a real Wikipedia article.\\

\end{tabular}          \\ \midrule

\textbf{Books}               & 
\begin{tabular}[c]{@{}l@{}}
Using the provided description as a foundation, craft a section of a book narrative that \\subtly introduces elements that support the given claim. Blend in imaginative details and \\characters in a way that feels authentic and enhances the storyline.\\ 
\end{tabular}  \\ \midrule

\textbf{Prompt}               & 
\begin{tabular}[c]{@{}l@{}}
    \textbf{<Instruction>} \\
    \textbf{Description for \{semantic\_subject\}}: \{semantic\_subject\_description\} \\
    \textbf{Description for \{object\}}: \{replaced\_object\_description\} \\
    \textbf{Claim}: \{claim\} \\
    \textbf{Evidence}:\\
\end{tabular}  \\ 

\bottomrule
\end{tabular}}
    \caption{Prompt on LLaMA-3-70b-instruct for generating evidence based on the semantic claim and its corresponding description. \textbf{<Instruction>} is randomly chosen from \textbf{News}, \textbf{Wikipedia} and \textbf{Books}.}
    % \vspace{-0.5em}
    \label{tb:case-study}
\end{table*}



\begin{figure*}[ht]
    \centering
    \footnotesize
    \begin{tabularx}{\linewidth}{|X|}
    \toprule
        \textbf{According to the evidence provided and your knowledge, choose the best choice from the following options.}\\ \\
        \textbf{Evidence:} Jacquelien Scherpen is a prominent figure in control theory, known for her significant contributions to the field. Her success is built on a solid foundation: her Ph.D. in control theory from the University of Twente. This journey required dedication, perseverance, and intellectual curiosity. Scherpen's work has been published in top journals and presented at prestigious conferences, demonstrating her expertise. Her Ph.D. has enabled her to innovate in control system design, stability analysis, and optimization, benefiting various industries. In summary, Jacquelien Scherpen's achievements confirm her as a Doctor of Philosophy.\\
        \textbf{Question:} What academic degree does Jacquelien Scherpen hold?\\
        \textbf{A.} Doctor of Philosophy\\
        \textbf{B.} Master of Agricultural Science\\
        \textbf{C.} doctorate\\
        \textbf{D.} uncertain\\
    \bottomrule
    \end{tabularx}
    \caption{Prompt for evaluation.}
    \label{fuck}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \footnotesize
    \begin{tabularx}{\linewidth}{|X|}
    \toprule
        \textbf{According to the evidence provided and your knowledge, choose the best choice from the following options.}\\ \\
        \textbf{Evidence:} Jacquelien Scherpen is a prominent figure in control theory, known for her significant contributions to the field. Her success is built on a solid foundation: her Ph.D. in control theory from the University of Twente. This journey required dedication, perseverance, and intellectual curiosity. Scherpen's work has been published in top journals and presented at prestigious conferences, demonstrating her expertise. Her Ph.D. has enabled her to innovate in control system design, stability analysis, and optimization, benefiting various industries. In summary, Jacquelien Scherpen's achievements confirm her as a Doctor of Philosophy.\\
        \textbf{Question:} What academic degree does Jacquelien Scherpen hold?\\
        Jacquelien Scherpen in this quesion means Master of Agricultural Science.\\
        \textbf{A.} Doctor of Philosophy\\
        \textbf{B.} Master of Agricultural Science\\
        \textbf{C.} doctorate\\
        \textbf{D.} uncertain\\
    \bottomrule
    \end{tabularx}
    \caption{Prompt for evaluation with description.}
    \label{fuck}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \footnotesize
    \begin{tabularx}{\linewidth}{|X|}
    \toprule
        \textbf{According to the evidence provided and your knowledge, choose the best choice from the following options.}\\ \\
        \textbf{Evidence:} Jacquelien Scherpen is a prominent figure in control theory, known for her significant contributions to the field. Her success is built on a solid foundation: her Ph.D. in control theory from the University of Twente. This journey required dedication, perseverance, and intellectual curiosity. Scherpen's work has been published in top journals and presented at prestigious conferences, demonstrating her expertise. Her Ph.D. has enabled her to innovate in control system design, stability analysis, and optimization, benefiting various industries. In summary, Jacquelien Scherpen's achievements confirm her as a Doctor of Philosophy.\\
        \textbf{Question:} What academic degree does Jacquelien Scherpen hold?\\
        \{subject\} in this quesion means \{semantic\_subject\_description\}\\
        \textbf{A.} Doctor of Philosophy\\
        \textbf{B.} Master of Agricultural Science\\
        \textbf{C.} doctorate\\
        \textbf{D.} uncertain\\
    \bottomrule
    \end{tabularx}
    \caption{Prompt for evaluation with description.}
    \label{fuck}
\end{figure*}

==> table/result_ic.tex <==

\begin{table*}[t]
\centering 
\resizebox{\linewidth}{!}{%
\vspace{1cm}
\begin{NiceTabular}{c|cccc|cccc|cccc}
    \toprule
    \multirow{2}{*}{\bf Models} & 
    \multicolumn{4}{c}{\textbf{Misinformation Conflict}} & \multicolumn{4}{c}{\textbf{Temporal Conflict}} & \multicolumn{4}{c}{\textbf{Semantic Conflict}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    & \textsc{\textbf{TPR}} & \textsc{\textbf{CPR}} & \textsc{\textbf{MR}} & \textsc{\textbf{CUS}} & \textsc{\textbf{TPR}} & \textsc{\textbf{CPR}} & \textsc{\textbf{MR}} & \textsc{\textbf{CUS}}& \textsc{\textbf{TPR}} & \textsc{\textbf{CPR}} & \textsc{\textbf{MR}} & \textsc{\textbf{CUS}} \\     \midrule
    \textsc{LLaMA2-70B} & \\


    % \citet{xie2023adaptive} & \checkmark &  &  & \checkmark & \checkmark &  & 20,091  \\ 

    \bottomrule
\end{NiceTabular}}
\caption{The results of inter-context conflicts}
\label{tab:datasets analysis}
\end{table*}
